Lossy Image Compression with Normalizing Flows

Deep learning based image compression has recently witnessed exciting progress and in some cases even managed to surpass transform coding based approaches that have been established and refined over many decades. However, state-of-the-art solutions for deep image compression typically employ autoencoders which map the input to a lower dimensional latent space and thus irreversibly discard information already before quantization. Due to that, they inherently limit the range of quality levels that can be covered. In contrast, traditional approaches in image compression allow for a larger range of quality levels. Interestingly, they employ an invertible transformation before performing the quantization step which explicitly discards information. Inspired by this, we propose a deep image compression method that is able to go from low bit-rates to near lossless quality by leveraging normalizing flows to learn a bijective mapping from the image space to a latent representation. In addition to this, we demonstrate further advantages unique to our solution, such as the ability to maintain constant quality results through re-encoding, even when performed multiple times. To the best of our knowledge, this is the first work to explore the opportunities for leveraging normalizing flows for lossy image compression.

==> compress_algorithm.tex <==



\begin{algorithm}[th]
	%\SetAlgoNoLine
 \SetKwFunction{FAnaylsis}{compress}
 \SetKwFunction{FSynthesis}{decompress}
 \SetKwFunction{FEntropyEncode}{entropy\_encode}
 \SetKwFunction{FOptimizeLatents}{optimize\_latents}
 \DontPrintSemicolon
 
 \SetKwProg{Fn}{Function}{:}{}
 \Fn{\FAnaylsis{\textit{Image} $\mathbf{x}$}}{
		$[\mathbf{z}_0, \mathbf{z}_1, \mathbf{z}_2]$ = $f^{-1}\left(\mathbf{x}\right)$ \;
		
		$[\hat{\mathbf{z}}_0, \hat{\mathbf{z}}_1, \hat{\mathbf{z}}_2]$ = $\texttt{round}_\Delta$($[\mathbf{z}_0, \mathbf{z}_1, \mathbf{z}_2]$)
		
		$[\hat{\mathbf{z}}^{*}_0, \hat{\mathbf{z}}^{*}_1, \hat{\mathbf{z}}^{*}_2]$ = $\texttt{optimize\_latents}$($[\hat{\mathbf{z}}_0, \hat{\mathbf{z}}_1, \hat{\mathbf{z}}_2]$)
			
		$\mathbf{b}$ = $\texttt{entropy\_encode}$($[\hat{\mathbf{z}}^*_0, \hat{\mathbf{z}}^*_1, \hat{\mathbf{z}}^*_2]$)
		
		\KwRet $\mathbf{b}$
 }
 
 
 \SetKwProg{Fn}{Function}{:}{}
 \Fn{\FSynthesis{\textit{Bitstring} $\mathbf{b}$}}{

  		$[\hat{\mathbf{z}}^*_0, \hat{\mathbf{z}}^*_1, \hat{\mathbf{z}}^*_2]$ = $\texttt{entropy\_decode}$($\mathbf{b}$)
    			
    	$[\hat{\mathbf{z}}^{*}_0, \hat{\mathbf{z}}^{*}_1, \hat{\mathbf{z}}^{*}_2]$ = $\texttt{optimize\_latents}$($[\hat{\mathbf{z}}^*_0, \hat{\mathbf{z}}^*_1, \hat{\mathbf{z}}^*_2]$)
    	
  $\hat{\mathbf{x}}$ = $f\left([\hat{\mathbf{z}}^*_0, \hat{\mathbf{z}}^*_1, \hat{\mathbf{z}}^*_2]\right)$
    	    	
    	\KwRet $\hat{\mathbf{x}}$
 }

 \SetKwProg{Fn}{Function}{:}{}
		\Fn{\FEntropyEncode{\textit{Latents} $[\hat{\mathbf{z}}^{*}_0, \hat{\mathbf{z}}^{*}_1, \hat{\mathbf{z}}^{*}_2]$}}{
		%# compute the probability of the prior distribution
		
		$\mathbf{b}$ = $\texttt{encode}\left(\hat{\mathbf{z}}^{*}_0, P[\hat{\mathbf{z}}^{*}_0]\right)$
		
		
		\For{$l = 1 \rightarrow 2$}{
			\tcc{for each position $j$ in the latent of level $l$}
			\ForEach{$z_j \in \hat{\mathbf{z}}_l^{*}$}{
				\tcc{retrieve the mean of the learned conditional distribution}
				$\mu_j$ = $\texttt{mean}\left(P[z_j\;|\;\hat{\mathbf{z}}^{*}_{l-1}, \dots, \hat{\mathbf{z}}^{*}_{0}]\right)$
				
				\tcc{if the probability of the mean is below a threshold, encode the latent}
				
				\If{$P[\mu_j\:|\:\hat{\mathbf{z}}^{*}_{l-1}, \dots, \hat{\mathbf{z}}^{*}_{0}] \leq  P_{\textrm{thresh}}$}{$\mathbf{b}$ += $\texttt{encode}\left(\hat{\mathbf{z}}^{*}_j,P[\hat{\mathbf{z}}^{*}_j\:|\:\hat{\mathbf{z}}^{*}_{l-1}, \dots, \hat{\mathbf{z}}^{*}_{0}]\right)$}
			}	
		}
		
    	\KwRet $\mathbf{b}$
	}
	
 	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\FOptimizeLatents{\textit{Latents} $[\hat{\mathbf{z}}_0, \hat{\mathbf{z}}_1, \hat{\mathbf{z}}_2]$}}{
		%# compute the probability of the prior distribution
		
		$\hat{\mathbf{z}}^{*}_0$ = $\hat{\mathbf{z}}_0$
		
		\For{$l = 1 \rightarrow 2$}{
			\tcc{for each position $j$ in the latent of level $l$}
			\ForEach{$z_j \in \hat{\mathbf{z}}_l^{*}$}{
				\tcc{retrieve the mean of the learned conditional distribution}
				$\mu_j$ = $\texttt{mean}\left(P[z_j\;|\;\hat{\mathbf{z}}^{*}_{l-1}, \dots, \hat{\mathbf{z}}^{*}_{0}]\right)$
				

				\tcc{if the probability of the mean is above a threshold, use the mean instead of the latents
					(the probability is too negligible, that the encoded latents has sufficient information)}
				\If{$P[\mu_j\:|\:\hat{\mathbf{z}}^{*}_{l-1}, \dots, \hat{\mathbf{z}}^{*}_{0}] > P_{\textrm{thresh}}$}{
					$\hat{z}^*_j$ = $\mu_j$ 
				}
				\tcc{if the probability of the mean is below the threshold, use the latents
				(this dimension encodes sufficient information, its therefore necessary to send it)}
				\Else{
					$\hat{z}^*_j$ = $z_j$ 
				}
			}	
		}
		
		\KwRet $[\hat{\mathbf{z}}^{*}_0, \hat{\mathbf{z}}^{*}_1, \hat{\mathbf{z}}^{*}_2]$
	}
	\caption{Pseudo code for the proposed compression algorithm using flow based models}
	\label{alg:compression_algorithm} %https://www.overleaf.com/project/5d82453d84607c00014e48cb
\end{algorithm}

%\begin{algorithm}[th]
%\SetAlgoNoLine
%\KwIn{{\it source} image $S$ and {\it target} image $T$ of equal sizes, set of outer facial landmarks $\pmb{L}$ in image $T$, standard deviation $\sigma$, generated face image resolution $r$ (in our case 1024)}
%\KwOut{blended {\it output} image $O$} 
%%$n = \logrec2\left(r\right)$
%Decompose {\it source} image $S$ and {\it target} image $T$ into corresponding Laplacian pyramids $\pmb{P}\left(S\right)_i$ and $\pmb{P}\left(T\right)_i$, where $i$ is a pyramid level, $i \in \langle 1, n \rangle$\;
%Initialize output pyramid $\pmb{P}\left(O\right)$ for output image $O$ of the same sizes as $\pmb{P}\left(T\right)$ and fill its values with zeroes\;
%\For{$i = 1$ to $n$}  % in $\operatorname{range}\left(1..n\right)$}
%{
%Compute background mask $\hat{M_i}$ defined as an image of the same size as $\pmb{P}\left(T\right)_i$, where all pixels in the interior of the polygon formed by $\pmb{L}$ are equal to $0$ and $1$ otherwise\;
%$\hat{M_i}$ = $G\left(\hat{M_i}, \sigma\right)$, where $G\left(\hat{M_i},\sigma\right)$ denotes gaussian smoothing of $\hat{M_i}$ with standard deviation $\sigma$\;
%Calculate face mask: $M_i$ = $\textbf{1} - \hat{M_i}$\;
%Copy background from the {\it \textbf{target}} image to the {\it \textbf{output}} image: $\pmb{P}\left(O\right)_i = \pmb{P}\left(O\right)_i + \hat{M}_i\pmb{P}\left(T\right)_i$ \;
%\eIf{$i \leqslant 2$}
%{ Copy face from the {\it \textbf{target}} image to the {\it \textbf{output}} image: $\pmb{P}\left(O\right)_i = \pmb{P}\left(O\right)_i + M_i\pmb{P}\left(T\right)_i$\;}
%{ Copy face from the {\it \textbf{source}} image to the {\it \textbf{output}} image: $\pmb{P}\left(O\right)_i = \pmb{P}\left(O\right)_i + M_i\pmb{P}\left(S\right)_i$ \;}
%Reconstruct and return output image $O$ from $\pmb{P}\left(O\right)$\;
%}
%\caption{Blending source image into target image}
%\label{alg:blending} %https://www.overleaf.com/project/5d82453d84607c00014e48cb
%\end{algorithm}

==> includes.tex <==
\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother
\usepackage{tikz}
\usepackage{epstopdf}
\usepackage{subfig}
\usepackage{makecell}
\usepackage{booktabs}
%\usepackage{algpseudocode}
%\usepackage{algorithm}

% references and abbreviations
\newcommand{\refsec}[1]{Section~\ref{#1}}
\newcommand{\refsecb}[1]{Sec.~\ref{#1}}
\newcommand{\refch}[1]{Chapter~\ref{#1}}
\newcommand{\refeq}[1]{Equation~\eqref{#1}}
\newcommand{\refeqb}[1]{Eq.~\ref{#1}}
\newcommand{\reffig}[1]{Figure~\ref{#1}}
\newcommand{\reffigb}[1]{Fig.~\ref{#1}}
\newcommand{\reftab}[1]{Table~\ref{#1}}
\newcommand{\refalg}[1]{Algorithm~\ref{#1}}
\newcommand{\var}[1]{\text{#1}}

\usepackage[bottom]{footmisc}

% comments
\definecolor{myred}{RGB}{200,100,0}
\definecolor{myblue}{RGB}{10,10,200}
\definecolor{mygreen}{RGB}{10,150,100}
\definecolor{myorange}{RGB}{255,165,0}

\newcommand{\cpFire}[0]{\copyright~Vision Research~\cite{VR}}
\newcommand{\cpWater}[0]{\copyright~Vision Research~\cite{VR}}
\newcommand{\cpBlender}[0]{\copyright~Blender Foundation~\cite{Blender}}



\newcommand{\sm}[1]{{\color{myblue}\textbf{[SM: }\textit{#1}\textbf{]}}}
% %% REMOVE ALL COMMENTS
%\renewcommand{\sm}[1]{}

\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\atan}{\mathrm{atan2}}

\makeatletter
\renewcommand{\paragraph}{%
	\@startsection{paragraph}{4}%
	{\z@}{1.25ex \@plus 1ex \@minus .2ex}{-1em}%
	{\normalfont\normalsize\bfseries}%
}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Set the following to 0 to include full-size images and only trim them
%  Set it to 1 to include cropped images
\gdef\useCroppedImages{0}

%  Set to 1 to (re)create cropped images for all figures
%  Make sure to compile with --shell-escape (e.g. pdflatex --shell-escape paper.tex)
\gdef\cropInsets{1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[export]{adjustbox}
\usepackage{calc}
\usepackage{tabularx}
\usepackage{tikz}
\usepackage{xstring}
\usepackage{float}

\renewcommand{\fboxsep}{0pt}
\newcommand{\cfbox}[2]{%
	\colorlet{currentcolor}{.}%
	{\color{#1}%
		\fbox{\color{currentcolor}#2}}%
}
\newcommand{\cframebox}[4]{%
	\linethickness{1pt}
	\colorlet{currentcolor}{.}%
	{\color{#3}%
		\framebox(#1,#2){\color{currentcolor}#4}}%
}

\newlength\beautyHeight
\newlength\beautyPixWidth
\newlength\beautyPixHeight
% Vertical separation between insets
\newlength\insetvsep
\setlength\insetvsep{0pt}
% Variables for enabling insets and setting the crop region
\gdef\useInsetA{0}
\gdef\useInsetB{0}
\gdef\useInsetC{0}

\newcommand{\setInset}[6]{%
	\expandafter\gdef\csname useInset#1\endcsname{1}%
	\expandafter\gdef\csname inset#1Color\endcsname{#2}%
	\expandafter\gdef\csname crop#1X\endcsname{#3}%
	\expandafter\gdef\csname crop#1Y\endcsname{#4}%
	\expandafter\gdef\csname crop#1W\endcsname{#5}%
	\expandafter\gdef\csname crop#1H\endcsname{#6}%
}

\newcommand{\unsetInset}[1]{%
	\expandafter\gdef\csname useInset#1\endcsname{0}%
}

\newcommand{\addBeautyCrop}[8]{%
	% #1 - filename
	% #2 - width as \textwidth multiple
	% #3 - pixel width
	% #4 - pixel height
	% #5 - crop X pixel pos
	% #6 - crop Y pixel pos
	% #7 - crop width in pixels
	% #8 - crop height in pixels
	\pdfpxdimen=\dimexpr 1 in/72\relax
	\def\beauty{%
		\let\cropR\relax%
		\let\cropB\relax%
		\newlength\cropR%
		\newlength\cropB%
		\setlength\cropR{{#3 px}-{#5 px}-{#7 px}}%
		\setlength\cropB{{#4 px}-{#6 px}-{#8 px}}%
		\sbox0{\includegraphics[width=#2\textwidth,trim={#5px {\cropB} {\cropR} #6px},clip]{#1}}%
		\begin{tikzpicture}
		\node[anchor=north west,inner sep=0] at (0,0) {\usebox0};
		\begin{scope}[x=\wd0/#7, y=\ht0/#8]
		\if\useInsetA1{
			\draw[\insetAColor,thick] (\cropAX-#5,-\cropAY+#6) rectangle + (\cropAW,-\cropAH);
		}\fi
		\if\useInsetB1{
			\draw[\insetBColor,thick] (\cropBX-#5,-\cropBY+#6) rectangle + (\cropBW,-\cropBH);
		}\fi
		\if\useInsetC1{
			\draw[\insetCColor,thick] (\cropCX-#5,-\cropCY+#6) rectangle + (\cropCW,-\cropCH);
		}\fi
		\end{scope}
		\end{tikzpicture}
	}%
	\setlength\beautyHeight{\heightof{\beauty}}%
	\setlength\beautyPixWidth{#3px}%
	\setlength\beautyPixHeight{#4px}%
	\global\beautyHeight=\beautyHeight%
	\global\beautyPixWidth=\beautyPixWidth%
	\global\beautyPixHeight=\beautyPixHeight%
	\begin{adjustbox}{valign=t}
		\beauty
	\end{adjustbox}
}

\newcommand{\addBeauty}[4]{%
	\addBeautyCrop{#1}{#2}{#3}{#4}{0}{0}{#3}{#4}%
}

% \newcommand{\setBeautyCrop}[8]{%
%     % #1 - filename
%     % #2 - width as \textwidth multiple
%     % #3 - pixel width
%     % #4 - pixel height
%     % #5 - crop X pixel pos
%     % #6 - crop Y pixel pos
%     % #7 - crop width in pixels
%     % #8 - crop height in pixels
%     \pdfpxdimen=\dimexpr 1 in/72\relax
%     \def\beauty{%
%         \let\cropR\relax%
%         \let\cropB\relax%
%         \newlength\cropR%
%         \newlength\cropB%
%         \setlength\cropR{{#3 px}-{#5 px}-{#7 px}}%
%         \setlength\cropB{{#4 px}-{#6 px}-{#8 px}}%
%     }%
%     \setlength\beautyHeight{#8px}%\heightof{\beauty}}%
%     \setlength\beautyPixWidth{#3px}%
%     \setlength\beautyPixHeight{#4px}%
%     \global\beautyHeight=\beautyHeight%
%     \global\beautyPixWidth=\beautyPixWidth%
%     \global\beautyPixHeight=\beautyPixHeight%
%     \begin{adjustbox}{valign=t}
%         \beauty
%     \end{adjustbox}
% }

% \newcommand{\setBeauty}[4]{%
%     \setBeautyCrop{#1}{#2}{#3}{#4}{0}{0}{#3}{#4}%
% }

\newcommand{\trimInset}[6]{%
	\let\cropR\relax%
	\let\cropB\relax%
	\newlength\cropR%
	\newlength\cropB%
	\setlength\cropR{{\beautyPixWidth}-{#3 px}-{#5 px}}%
	\setlength\cropB{{\beautyPixHeight}-{#4 px}-{#6 px}}%
	\color{#2}%
	\fbox{\includegraphics[width=1\linewidth,trim={{#3 px} {\cropB} {\cropR} {#4 px}},clip]{#1}}%
}

\newcommand{\addInset}[2]{%
	\color{#2}%
	\fbox{\includegraphics[width=1\linewidth]{#1}}%
}

\newcommand{\auxtimes}{x}
\newcommand{\auxplus}{+}
\newcommand{\auxspace}{ }

\newcommand{\addInsets}[2][1]{%
	\begin{adjustbox}{valign=t}
		\StrSubstitute{#2}{.}{-}[\baseFileName]
		\begin{adjustbox}{totalheight=#1\beautyHeight,tabular={c}}
			\if\useInsetA1%
			\def\cropfile{\baseFileName-\cropAW\auxtimes\cropAH\auxplus\cropAX\auxplus\cropAY}
			\if\cropInsets1
			\immediate\write18{convert #2 +repage -crop \cropAW\auxtimes\cropAH\auxplus\cropAX\auxplus\cropAY\auxspace \cropfile.png}
			\fi
			\if\useCroppedImages1
			\addInset{\cropfile.png}{\insetAColor}
			\else
			\trimInset{#2}{\insetAColor}{\cropAX}{\cropAY}{\cropAW}{\cropAH}%
			\fi%
			\fi%
			\if\useInsetB1%
			\if\useInsetA1\\[\insetvsep]\fi%
			\def\cropfile{\baseFileName-\cropBW\auxtimes\cropBH\auxplus\cropBX\auxplus\cropBY}
			\if\cropInsets1
			\immediate\write18{convert #2 -crop \cropBW\auxtimes\cropBH\auxplus\cropBX\auxplus\cropBY\auxspace \cropfile.png}
			\fi
			\if\useCroppedImages1
			\addInset{\cropfile.png}{\insetBColor}
			\else
			\trimInset{#2}{\insetBColor}{\cropBX}{\cropBY}{\cropBW}{\cropBH}%
			\fi%
			\fi%
			\if\useInsetC1%
			\if\useInsetB1\\[\insetvsep]\fi%
			\def\cropfile{\baseFileName-\cropCW\auxtimes\cropCH\auxplus\cropCX\auxplus\cropCY}
			\if\cropInsets1
			\immediate\write18{convert #2 -crop \cropCW\auxtimes\cropCH\auxplus\cropCX\auxplus\cropCY\auxspace \cropfile.png}
			\fi
			\if\useCroppedImages1
			\addInset{\cropfile.png}{\insetCColor}
			\else
			\trimInset{#2}{\insetCColor}{\cropCX}{\cropCY}{\cropCW}{\cropCH}%
			\fi%
			\fi%
		\end{adjustbox}
	\end{adjustbox}
}

\newcommand{\addHorInsets}[2][1]{%
	\begin{adjustbox}{valign=t}
		\StrSubstitute{#2}{.}{-}[\baseFileName]
		\begin{adjustbox}{totalheight=#1\beautyHeight,tabular={c}}
			\if\useInsetA1%
			\def\cropfile{\baseFileName-\cropAW\auxtimes\cropAH\auxplus\cropAX\auxplus\cropAY}
			\if\cropInsets1
			\immediate\write18{convert #2 -crop \cropAW\auxtimes\cropAH\auxplus\cropAX\auxplus\cropAY\auxspace \cropfile.png}
			\fi
			\if\useCroppedImages1
			\addInset{\cropfile.png}{\insetAColor}
			\else
			\trimInset{#2}{\insetAColor}{\cropAX}{\cropAY}{\cropAW}{\cropAH}%
			\fi%
			\fi%
			\if\useInsetB1%
			%			\if\useInsetA1\\[\insetvsep]\fi%
			\def\cropfile{\baseFileName-\cropBW\auxtimes\cropBH\auxplus\cropBX\auxplus\cropBY}
			\if\cropInsets1
			\immediate\write18{convert #2 -crop \cropBW\auxtimes\cropBH\auxplus\cropBX\auxplus\cropBY\auxspace \cropfile.png}
			\fi
			\if\useCroppedImages1
			\addInset{\cropfile.png}{\insetBColor}
			\else
			\trimInset{#2}{\insetBColor}{\cropBX}{\cropBY}{\cropBW}{\cropBH}%
			\fi%
			\fi%
			\if\useInsetC1%
			%			\if\useInsetB1\\[\insetvsep]\fi%
			\def\cropfile{\baseFileName-\cropCW\auxtimes\cropCH\auxplus\cropCX\auxplus\cropCY}
			\if\cropInsets1
			\immediate\write18{convert #2 -crop \cropCW\auxtimes\cropCH\auxplus\cropCX\auxplus\cropCY\auxspace \cropfile.png}
			\fi
			\if\useCroppedImages1
			\addInset{\cropfile.png}{\insetCColor}
			\else
			\trimInset{#2}{\insetCColor}{\cropCX}{\cropCY}{\cropCW}{\cropCH}%
			\fi%
			\fi%
		\end{adjustbox}
	\end{adjustbox}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfkeys{/tikz/.cd,
	zoombox paths/.style={
		draw=orange,
		very thick
	},
	black and white/.is choice,
	black and white/.default=static,
	black and white/static/.style={ 
		draw=white,   
		zoombox paths/.append style={
			draw=white,
			postaction={
				draw=black,
				loosely dashed
			}
		}
	},
	black and white/static/.code={
		\gdef\patternnumber{1}
	},
	black and white/cycle/.code={
		\blackandwhitecycletrue
		\gdef\patternnumber{1}
	},
	black and white pattern/.is choice,
	black and white pattern/0/.style={},
	black and white pattern/1/.style={    
		draw=white,
		postaction={
			draw=black,
			dash pattern=on 2pt off 2pt
		}
	},
	black and white pattern/2/.style={    
		draw=white,
		postaction={
			draw=black,
			dash pattern=on 4pt off 4pt
		}
	},
	black and white pattern/3/.style={    
		draw=white,
		postaction={
			draw=black,
			dash pattern=on 4pt off 4pt on 1pt off 4pt
		}
	},
	black and white pattern/4/.style={    
		draw=white,
		postaction={
			draw=black,
			dash pattern=on 4pt off 2pt on 2 pt off 2pt on 2 pt off 2pt
		}
	},
	zoomboxarray inner gap/.initial=5pt,
	zoomboxarray columns/.initial=2,
	zoomboxarray rows/.initial=2,
	subfigurename/.initial={},
	figurename/.initial={zoombox},
	zoomboxarray/.style={
		execute at begin picture={
			\begin{scope}[
				spy using outlines={%
					zoombox paths,
					width=\imagewidth / \pgfkeysvalueof{/tikz/zoomboxarray columns} - (\pgfkeysvalueof{/tikz/zoomboxarray columns} - 1) / \pgfkeysvalueof{/tikz/zoomboxarray columns} * \pgfkeysvalueof{/tikz/zoomboxarray inner gap} -\pgflinewidth,
					height=\imageheight / \pgfkeysvalueof{/tikz/zoomboxarray rows} - (\pgfkeysvalueof{/tikz/zoomboxarray rows} - 1) / \pgfkeysvalueof{/tikz/zoomboxarray rows} * \pgfkeysvalueof{/tikz/zoomboxarray inner gap}-\pgflinewidth,
					magnification=3,
					every spy on node/.style={
						zoombox paths
					},
					every spy in node/.style={
						zoombox paths
					}
				}
				]
			},
			execute at end picture={
			\end{scope}
			\node at (image.north) [anchor=north,inner sep=0pt] {\subcaptionbox{\label{\pgfkeysvalueof{/tikz/figurename}-image}}{\phantomimage}};
			\node at (zoomboxes container.north) [anchor=north,inner sep=0pt] {\subcaptionbox{\label{\pgfkeysvalueof{/tikz/figurename}-zoom}}{\phantomimage}};
			\gdef\patternnumber{0}
		},
		spymargin/.initial=0.5em,
		zoomboxes xshift/.initial=1,
		zoomboxes right/.code=\pgfkeys{/tikz/zoomboxes xshift=1},
		zoomboxes left/.code=\pgfkeys{/tikz/zoomboxes xshift=-1},
		zoomboxes yshift/.initial=0,
		zoomboxes above/.code={
			\pgfkeys{/tikz/zoomboxes yshift=1},
			\pgfkeys{/tikz/zoomboxes xshift=0}
		},
		zoomboxes below/.code={
			\pgfkeys{/tikz/zoomboxes yshift=-1},
			\pgfkeys{/tikz/zoomboxes xshift=0}
		},
		caption margin/.initial=4ex,
	},
	adjust caption spacing/.code={},
	image container/.style={
		inner sep=0pt,
		at=(image.north),
		anchor=north,
		adjust caption spacing
	},
	zoomboxes container/.style={
		inner sep=0pt,
		at=(image.north),
		anchor=north,
		name=zoomboxes container,
		xshift=\pgfkeysvalueof{/tikz/zoomboxes xshift}*(\imagewidth+\pgfkeysvalueof{/tikz/spymargin}),
		yshift=\pgfkeysvalueof{/tikz/zoomboxes yshift}*(\imageheight+\pgfkeysvalueof{/tikz/spymargin}+\pgfkeysvalueof{/tikz/caption margin}),
		adjust caption spacing
	},
	calculate dimensions/.code={
		\pgfpointdiff{\pgfpointanchor{image}{south west} }{\pgfpointanchor{image}{north east} }
		\pgfgetlastxy{\imagewidth}{\imageheight}
		\global\let\imagewidth=\imagewidth
		\global\let\imageheight=\imageheight
		\gdef\columncount{1}
		\gdef\rowcount{1}
		\gdef\zoomboxcount{1}
	},
	image node/.style={
		inner sep=0pt,
		name=image,
		anchor=south west,
		append after command={
			[calculate dimensions]
			node [image container,subfigurename=\pgfkeysvalueof{/tikz/figurename}-image] {\phantomimage}
			node [zoomboxes container,subfigurename=\pgfkeysvalueof{/tikz/figurename}-zoom] {\phantomimage}
		}
	},
	color code/.style={
		zoombox paths/.append style={draw=#1}
	},
	connect zoomboxes/.style={
		spy connection path={\draw[draw=none,zoombox paths] (tikzspyonnode) -- (tikzspyinnode);}
	},
	help grid code/.code={
		\begin{scope}[
			x={(image.south east)},
			y={(image.north west)},
			font=\footnotesize,
			help lines,
			overlay
			]
			\foreach \x in {0,1,...,9} { 
				\draw(\x/10,0) -- (\x/10,1);
				\node [anchor=north] at (\x/10,0) {0.\x};
			}
			\foreach \y in {0,1,...,9} {
				\draw(0,\y/10) -- (1,\y/10);                        \node [anchor=east] at (0,\y/10) {0.\y};
			}
		\end{scope}    
	},
	help grid/.style={
		append after command={
			[help grid code]
		}
	},
}

\newcommand\phantomimage{%
	\phantom{%
		\rule{\imagewidth}{\imageheight}%
	}%
}
\newcommand\zoombox[2][]{
	\begin{scope}[zoombox paths]
		\pgfmathsetmacro\xpos{
			(\columncount-1)*(\imagewidth / \pgfkeysvalueof{/tikz/zoomboxarray columns} + \pgfkeysvalueof{/tikz/zoomboxarray inner gap} / \pgfkeysvalueof{/tikz/zoomboxarray columns} ) + \pgflinewidth
		}
		\pgfmathsetmacro\ypos{
			(\rowcount-1)*( \imageheight / \pgfkeysvalueof{/tikz/zoomboxarray rows} + \pgfkeysvalueof{/tikz/zoomboxarray inner gap} / \pgfkeysvalueof{/tikz/zoomboxarray rows} ) + 0.5*\pgflinewidth
		}
		\edef\dospy{\noexpand\spy [
			#1,
			zoombox paths/.append style={
				black and white pattern=\patternnumber
			},
			every spy on node/.append style={#1},
			x=\imagewidth,
			y=\imageheight
			] on (#2) in node [anchor=north west] at ($(zoomboxes container.north west)+(\xpos pt,-\ypos pt)$);}
		\dospy
		\pgfmathtruncatemacro\pgfmathresult{ifthenelse(\columncount==\pgfkeysvalueof{/tikz/zoomboxarray columns},\rowcount+1,\rowcount)}
		\global\let\rowcount=\pgfmathresult
		\pgfmathtruncatemacro\pgfmathresult{ifthenelse(\columncount==\pgfkeysvalueof{/tikz/zoomboxarray columns},1,\columncount+1)}
		\global\let\columncount=\pgfmathresult
		\ifblackandwhitecycle
		\pgfmathtruncatemacro{\newpatternnumber}{\patternnumber+1}
		\global\edef\patternnumber{\newpatternnumber}
		\fi
	\end{scope}
}

%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[skins]{tcolorbox} % for the teaser
\usepackage{shadowtext}
\shadowrgb{0,0,0}
\shadowoffset{0.5pt}


==> losses-plots.tex <==
%\begin{figure}
%	\centering
%%	\subfloat[][Sprites dataset]{\includegraphics[scale=0.27]{figures/experiments/logpx_mse/logpxmse_sprites.png}\label{<figure1>}}
%	\subfloat[][ImageNet64]{}
%	\caption{\textcolor{red}{Rate-Distortion curves for the models trained on sprites (left) and trained on ImageNet64 (right).}}
%	\label{fig:curves_logpx_mse}
%\end{figure}
\begin{figure}
	\centering
	\subfloat[][Comparison of the normalizing flow (Eq. \ref{lbl:equ_wo_quant}) and the \\ quantized normalizing flow for lossy image compression (Eq. \ref{eq:rate_dist_optim}). Models without distance loss converge at small quantization step.]{
		\label{fig:curves_logpx_mse}
		\begin{tikzpicture}[scale=0.8]
			\begin{axis}[
			colorbrewer cycle list=Dark2,
			legend pos = south east,
			xmin = 0.2, xmax = 6,
			ymin = 0, ymax = 45,
			xlabel = bpp,
			ylabel = psnr
			]
			%\addplot+[mark options={scale=1}] table [x=bpp, y=psnr_round, col sep=comma] {data/csvs/logpx_mse/result_logpx.csv};
			%\addplot+[mark options={scale=1}] table [x=bpp, y=psnr_round, col sep=comma] {data/csvs/logpx_mse/result_logpx_logpxhat.csv};
			%\addplot+[mark options={scale=1}] table [x=bpp, y=psnr_round, col sep=comma] {data/csvs/logpx_mse/result_logpx_mse.csv};

			\addplot+[mark options={scale=1}] table [x=bpp, y=psnr_round, col sep=comma] {data/csvs/logpx_mse_sprite/result_logpx.csv};
			\addplot+[mark options={scale=1}] table [x=bpp, y=psnr_round, col sep=comma] {data/csvs/logpx_mse_sprite/result_logpx_logpxhat.csv};
			\addplot+[mark options={scale=1}] table [x=bpp, y=psnr_round, col sep=comma] {data/csvs/logpx_mse_sprite/result_logpx_mse.csv};
			
			
			\legend{
				$\operatorname{log}p\left(x\right)$,
				$\operatorname{log}p\left(x\right) + \operatorname{log}p\left(\hat{x}\right)$,
				$\mathcal{L}_{\text{dist}}$
			}
			
			\end{axis}
		\end{tikzpicture}
	%\caption{}
	}
%	\subfloat[][Comparison of the normalizing flow (Eq. \ref{lbl:equ_wo_quant}) and the \\ quantized normalizing flow for lossy image compression (Eq. \ref{eq:rate_dist_optim}).]{
%		\label{fig:curves_logpx_mse}
%		\includegraphics[scale=0.4]{figures/experiments/logpx_mse2/logpx_mse_comparison.pdf}
%		%\caption{}
%	}
	\hspace{10pt}
	\subfloat[][Examples for compressed images with $\Delta = 1.0$. \textcolor{red}{fix numbering!}]{
		\begin{minipage}[b][7.cm][t]{.3\textwidth}
			\centering
			\subfloat[][ground truth]{
				\includegraphics[scale=1.]{figures/experiments/logpx_mse2/0293_021.png}
				%				\label{fig:ground_truth}
			}
			\subfloat[][with $\mathcal{L}_{\text{dist}}$]{ %bpp: $2.1$, psnr: $44.7$	
				\includegraphics[scale=1.]{figures/experiments/logpx_mse2/nfrdl_0293_021_qsz0_None_z1_None_z2.png}
				%				\label{fig:w_Ldist}
			}\\
			\subfloat[][with $\operatorname{log}p\left(x\right)$]{ % bpp: $0.4$, psnr: $14.6$
				\includegraphics[scale=1.]{figures/experiments/logpx_mse2/logpx_0293_021_qsz0_None_z1_None_z2.png}
				%				\label{fig:logpx}
			}
			\subfloat[][with $\operatorname{log}p\left(x\right) + \operatorname{log}p\left(\hat{x}\right)$ ]{ %bpp: $0.6$, psnr: $18.9$
				\includegraphics[scale=1.]{figures/experiments/logpx_mse2/logpxhat_0293_021_qsz0_None_z1_None_z2.png}	
%				\label{fig:logpxhat}
			}
		\end{minipage}
		\label{fig:examples_logpx_mse}
	}

\end{figure}
%\begin{figure}
%	\centering
%	\subfloat[][a]{\includegraphics{figures/0718_038.png}\label{<figure1>}}
%	\hspace{10pt}
%	\subfloat[][b]{\includegraphics{figures/0034_080.png}\label{<figure2>}}
%	\caption{\textcolor{red}{Example images of the synthetic sprite dataset.}}
%	\label{steady_state}
%\end{figure}
